Resilient Distributed Diffusion in Networks with Adversaries

In this paper, we study resilient distributed diffusion for multi-task estimation in the presence of adversaries where networked agents must estimate distinct but correlated states of interest by processing streaming data. We show that in general diffusion strategies are not resilient to malicious agents that do not adhere to the diffusion-based information processing rules. In particular, by exploiting the adaptive weights used for diffusing information, we develop time-dependent attack models that drive normal agents to converge to states selected by the attacker. We show that an attacker that has complete knowledge of the system can always drive its targeted agents to its desired estimates. Moreover, an attacker that does not have complete knowledge of the system including streaming data of targeted agents or the parameters they use in diffusion algorithms, can still be successful in deploying an attack by approximating the needed information. The attack models can be used for both stationary and non-stationary state estimation.In addition, we present and analyze a resilient distributed diffusion algorithm that is resilient to any data falsification attack in which the number of compromised agents in the local neighborhood of a normal agent is bounded. The proposed algorithm guarantees that all normal agents converge to their true target states if appropriate parameters are selected. We also analyze trade-off between the resilience of distributed diffusion and its performance in terms of steady-state mean-square-deviation (MSD) from the correct estimates. Finally, we evaluate the proposed attack models and resilient distributed diffusion algorithm using stationary and non-stationary multi-target localization.

==> 1.introduction.tex <==


%==================== Section : Introduction ========================
\section {Introduction}
% Motivation
Diffusion Least-Mean Squares (DLMS) is a powerful algorithm for distributed state estimation \cite{journals/spm/SayedTCZT13}. It enables networked agents to interact with neighbors to process streaming data and diffuse information across the network to perform the estimation tasks. Compared to a centralized approach, distributed diffusion offers multiple advantages \textcolor{green}{including} robustness to drifts in the statistical properties of the data, scalability, \textcolor{green}{reliance} on local data, and fast response among others. Applications of distributed diffusion include spectrum sensing in cognitive networks \cite{7086338}, target localization \cite{targetLocalization}, distributed clustering \cite{6232902}, and biologically inspired designs for mobile networks \cite{mobileAdaptiveNetworks}. 

\textcolor{revision}{Different than consensus-based distributed algorithms that often require a careful design of the underlying network topology in order to cope with byzantine attacks \cite{DBLP:journals/jsac/LeBlancZKS13} and random links \cite{4536069}},
diffusion strategies are known to be robust to node and link failures \textcolor{green}{as well as to} high noise levels
\textcolor{revision2}{\cite{6197748, 5948418, 7547395,6726166}}.
%\textcolor{revision}{\cite{6197748, 5948418, 7472545,6726166}}.
\textcolor{revision}{
However, a single adversary with a fixed different state will make the diffusion network fail to converge to its actual state. }
Resilience of diffusion-based distributed algorithms in the presence of  \textcolor{revision}{fixed-value Byzantine attacks} has been studied in \textcolor{revision}{\cite{journals/spm/SayedTCZT13,6232902}}. A general approach to counteract such attacks is to \textcolor{green}{allow agents within the network to fuse information collected from other agents in local neighborhoods using adaptive \textcolor{revision}{ instead of fixed combination rules (weights).
By doing so, only neighbors estimating a similar state will be assigned large weight so as to eliminate the influence of a fixed-value Byzantine adversary.
} }
%This approach improves resilience of the overall system, however, adaptive weights also introduce other  vulnerabilities within the network.}

% Problem
In this paper, we consider distributed diffusion for multi-task estimation where networked agents must estimate distinct, but correlated states of interest by processing streaming data. 
\textcolor{revision}{
Agents are designed to adopt adaptive weights when diffusing information with neighbors since adaptive weights exhibit better resilience than fixed weights to fixed-value byzantine adversaries and have been successfully applied to  multi-task distributed estimation and intruder problems. However, w}e are interested in understanding if adaptive weights introduce vulnerabilities that can be exploited by  \textcolor{revision}{byzantine adversaries of another type, e.g., time-dependent attack}. 
\textcolor{revision}{The first problem we consider is to analyze if it is possible for an attacker to compromise a node, and make other nodes in its neighborhood converge to a state selected by the attacker. Then, we consider a network attack and determine a minimum set of nodes to compromise to make all nodes within the network converge to attacker's desired state. As a result, we show that DLMS, which was considered to be resilient against Byzantine agents by itself (\cite{journals/spm/SayedTCZT13, 6232902,5948418}), is in fact, not resilient against time-dependent byzantine attack and can be manipulated by an adversarial attacker.} %We highlight that by the first time, our work dispels the myth that baseline diffusion multi-task LMS by itself is resilient to adversarial attack, as indicated by \cite{journals/spm/SayedTCZT13, 6232902,5948418}.}
\textcolor{revision}{
Adaptive weights, on the one hand, improves the resilience of diffusion algorithms to fixed-value Byzantine attacks, yet on the other hand, introduces vulnerabilities to time-dependent attacks.
It is a must that we keep adaptive weights in order to achieve resilience to fixed-value Byzantine attacks, yet we want to also add  resilience to time-dependent attacks.}


We know that without cooperation, all nodes can estimate their states with a known error as measured by the mean-square-deviation (MSD) \cite{journals/spm/SayedTCZT13}. However, nodes can do better if they cooperate and utilize the information collected from others while computing their own estimates. 
%In fact, they do $N$ times better \textcolor{green}{(in terms of MSD)} than without the cooperation. 
However, if there is even a single compromised node due to an attack, it can drive its neighbors' estimates to a desired value. \textcolor{green}{Thus, cooperation is good on the one hand when there is no attack, but on the other hand could be adverse even if one of the nodes is compromised. We analyze this issue in detail and we propose a resilient diffusion algorithm that performs better than the non-cooperative case even in the presence of adversarial nodes. It should be noted that we do not rely on detection methods to improve resilience because distributed detection with only local information may lead to false alarms \cite{6545301}.}

\textcolor{revision}{It is common to assume a strong attacker when examining the resilience of a distributed network \cite{DBLP:journals/jsac/LeBlancZKS13, mitra2016secure, DBLP:conf/amcc/ChenKM18}. 
And it is not hypothetical for modern attackers to gather a complete information of the system and to stealthily compromise the sensors/controllers through cyber means, Stuxnet \cite{5772960} as a good example.
In this paper, the attack model is also based on the assumption of a strong knowledge of the system. 
Yet we show that without such knowledge, the attacker can approximate it alternatively and succeed if the approximation is of good accuracy.}


Distributed optimization and estimation can also be performed using consensus algorithms. Resilience of consensus-based distributed algorithms in the presence of cyber attacks has received considerable attention recently, for instance see \textcolor{revision}{\cite{5779706, DBLP:journals/jsac/LeBlancZKS13,6736104, 7822915,abbas2018improving, yuanchen/AdversaryDetection}.} \textcolor{green}{In such problems,} it is typically assumed that the goal of attacker is to disrupt the convergence (stability) of the distributed algorithm. In contrast, this paper focuses on attacks that do not disrupt convergence, but drive normal agents to converge to states selected by the attacker, \textcolor{yellow}{which can be used for deception attacks that are more challenging than just disrupting convergence.}


%Contribution
The contributions of the paper are:
\begin{enumerate}
\item By exploiting the adaptive weights \textcolor{revision}{that aim to cope with fixed-value Byzantine attacks}, we develop \textcolor{revision}{time-dependent} attack models that drive normal agents to converge to states selected by an attacker. The attack models can be used to deceive a specific node or the entire network and are applicable to both stationary and non-stationary state estimation.
\textcolor{revision}{
Although the attack models are based on a strong knowledge of the system, we show the attack can also succeed without such knowledge to demonstrate the practicality of the proposed attack.
This for the first time dispels the myth that baseline diffusion multi-task LMS by itself is resilient to adversarial attack.}

\item We develop a resilient distributed diffusion algorithm \textcolor{revision}{that can achieve resilience to up to $F$ compromised nodes in one normal agent's neighborhood.}
% under the assumption that the number of compromised nodes in the neighborhood of each normal node is bounded by $F$.
\textcolor{green}{By selecting an appropriate $F$, the proposed algorithm guarantees normal agents will converge to their actual targets under any data falsification attacks.
%ensures that compromised nodes are not able to drive normal nodes to incorrect estimates. 
If the parameter $F$ selected by the normal agents is large,  the resilient distributed diffusion algorithm degenerates to non-cooperative estimation. Thus, we also analyze trade-off between the resilience of distributed diffusion and its performance degradation in terms of MSD.}


\item We evaluate the proposed attack models and the resilient estimation algorithm using both stationary and non-stationary multi-target localization. The simulation results are consistent with our theoretical analysis and show that the approach provides resilience to attacks while incurring performance degradation which depends on the assumption about the number of compromised nodes. 
\end{enumerate}

%Organization
The rest of the paper is organized as follows: Section \ref{preliminaries} briefly introduces distributed diffusion. Section \ref{sec:problem} presents the attack and resilient distributed diffusion problems. The single node and network attack models are presented in Sections \ref{the section of attack model} and \ref{the section of network attack model} respectively. Section \ref{sec:resilient_diffusion} presents and analyzes the resilient distributed diffusion algorithm.
Section \ref{sec:evaluation} presents simulation results evaluating our approach for multi-target localization. 
\textcolor{revision}{
Section \ref{sec:weak attack} discuss how to deploy the proposed attack in practice without strong knowledge of the system and presents the simulation results.}
Section \ref{sec:related_work} gives a brief overview of the related work and Section \ref{sec:con} concludes the paper.

==> Acknowledgments.tex <==

%-------------------- Acknowledgemets --------------------
\section{Acknowledgments}
This work is supported in part by the National Science Foundation (CNS-1238959), the Air Force Research Laboratory (FA 8750-14-2-0180), and by NIST (70NANB18H198). Any options, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of AFRL, NSF and NIST.

